Programming Puzzles

We introduce a new type of programming challenge called programming puzzles, as an objective and comprehensive evaluation of program synthesis, and release an open-source dataset of Python Programming Puzzles (P3). Each puzzle is defined by a short Python program $f$, and the goal is to find an input which makes $f$ return True. The puzzles are objective in that each one is specified entirely by the source code of its verifier $f$, so evaluating $f$ is all that is needed to test a candidate solution. They do not require an answer key or input/output examples, nor do they depend on natural language understanding. The dataset is comprehensive in that it spans problems of a range of difficulties and domains, ranging from trivial string manipulation problems, to classic programming puzzles (e.g., Tower of Hanoi), to interview/competitive-programming problems (e.g., dynamic programming), to longstanding open problems in algorithms and mathematics (e.g., factoring). We develop baseline enumerative program synthesis, GPT-3 and Codex solvers that are capable of solving puzzles -- even without access to any reference solutions -- by learning from their own past solutions. Codex performs best, solving up to 18% of 397 test problems with a single try and 80% of the problems with 1,000 tries per problem. In a small user study, we find a positive correlation between puzzle-solving performance and coding experience, and between the puzzle difficulty for humans and AI solvers. Therefore, further improvements on P3 could have a significant impact on many program synthesis areas.

==> ignore/macros.tex <==
\usepackage[notes=true, done=false, later=true, ]{dtrt}

\newcommand{\tal}[1]{\dtcolornote[Tal]{blue}{#1}}
\newcommand{\adam}[1]{\dtcolornote[Adam]{orange}{#1}}

\lstset{
    basicstyle = \small\ttfamily,
    stringstyle = \color{Brown},
    keywordstyle = \bfseries\color{MediumBlue},
    commentstyle = \itshape\rmfamily\color{Green},
    showstringspaces = false,
    columns = flexible,
	breaklines = true,
	texcl = true,
	mathescape = true,
    tabsize = 4,
    keepspaces = true
}

\newcommand\pyline[1]{\lstinline[language=Python,basicstyle=\ttfamily]{#1}}
\lstnewenvironment{pyblock}{\lstset{language=Python,frame=single,basicstyle=\ttfamily}}{}

\newcommand{\thedataset}{\textsc{P}y\textsc{ProP}\xspace}
\newcommand{\puzzle}{\textsc{ProP}\xspace}
\newcommand{\puzzles}{\puzzle{}s\xspace}

% PyREACH / PROP (programming puzzles) / PP / ...

==> ignore/old_scraps_ignore.tex <==


We introduce a large dataset of \textit{Programming Puzzles} (PPs). 
There have been a number of datasets proposed for programming, mathematical reasoning, and 

which is not the case for theorem-proving or SAT-solving datasets\footnote{Mathematicians outperform computers at proving theorems in English, but they do not outperform computers at the problem of generating machine-verifiable proofs which are often extremely long.}.

This is also the case of many theorem-proving and SAT-solving datasets.
We note that property 


==> ignore/sections/app.tex <==
\section{Mathematical puzzles}

\subsection{Geometry puzzles}


\subsubsection{Open problem: Kissing numbers}

\subsection{Graph theory problems}

\subsubsection{Regular graphs}
TBA
% http://www.maths.gla.ac.uk/~es/srgraphs.php
% https://www.win.tue.nl/~aeb/graphs/srg/srgtab.html

\subsubsection{Open problem: Conway 99-problem}

In 2014, John Conway offered \$1,000 for a solution to this problem dating back to \cite{norman96} as cited by \cite{wikiConway}. The problem asks, ``Is there a graph with 99 vertices in which every edge (i.e. pair of joined vertices) belongs to a unique triangle and every nonedge (pair of unjoined vertices) to a unique quadrilateral?'' which can be encoded in two lines of Python. The problem remains unsolved.%\footnote{Due to Conway's recent death, the author's of the present paper offer \$1,000 on his behalf for a solution to the problem.}

\section{Number theory puzzles}


\subsection{Four squares}
Given a non-negative integer $n$, a classic theorem of Lagrange says that $n$ can be written as the sum of four integer squares. The problem here is to find them. 
This is a challenging problem for numbers with tens of digits or more. We provide a elementary $\tilde{O}(n)$ solution: it firsts computes the set,
$$S=\{i^2+j^2\mid i,j \leq \sqrt{n}\}.$$ 
It then tests to see if, for any number $m \in S$, $n-m \in S$ using hashing. The known polynomial-time algorithms (poly-log$(n)$ time since the length of $n$ is $\log(n)$) involve fairly sophisticated techniques from number
theory or ``Hurwitz quaternions'' \cite{rabin1986randomized}.


\subsection{Open problem: RSA Challenge (Factoring)}

\subsection{Discrete log}

\subsubsection{blah}

\subsection{Further number theory problems}

\subsection{Probability problems}

It is not clear how to concisely check the answer to a probability puzzle of the form \textit{what is the probability of X?}. This can be done with a  \textit{slow check}--the checker computes the answer slowly (either exactly or  approximately with Monte Carlo sampling) while the solver is time-constrained as always. Thus it is an instance of a \textit{speedup problem} described earlier. This is illustrated with classic problems.

\subsubsection{The ballot problem}
In the Bertrand's Ballot problem \citep{bertrand1887}, there is an election between two candidates, where Candidate 1 receives $n_1$ votes and candidate 2 receives $n_2$ votes. The question is, \textit{for given $n_1, n_2$, what is the probability that if votes are counted in a random order, that Candidate 1 is strictly ahead of Candidate 2 during the entire counting}? We provide two checkers. They both compare the answer provided by the solver to a ground truth answer that is computed slowly. The first checker computes the probability exactly by by summing over the $(n_1+n_2)!$ permutations. The second checker approximates it by Monte Carlo sampling, and thus a greater error tolerance is provided. 

Using a nontrivial mathematical argument, \cite{bertrand1887} showed that the answer is exactly:
$$\frac{\max(n_1-n_2, 0)}{n_1+n_2}.$$
As discussed earlier, it may be much easier to solve this problem by ``finding the pattern'' rather than deriving the above formula from scratch. In particular, since the checker is glass-box, one may run the probability computation for small $n_1, n_2$ and identifying the above rule which can then be used to quickly solve problems for larger values.

We also consider an inverse problem in which the goal is to find $n_1$ and $n_2$ such that the target approximates a given probability in $[0,1]$.

\subsubsection{The birthday paradox}

==> ignore/sections/conclusion.tex <==
\section{Conclusions}

To conclude, we present a novel programming challenges dataset with the following desirable properties:
%: [general NP-complete, objective, easily extensible, abstract, requires no specialized language beyond python].


==> ignore/sections/dataset.tex <==
\section{The \thedataset Dataset}

\subsection{Creation process}
The following sources were used for identifying possible \puzzle{}s. 
\begin{itemize}
    \item Wikipedia, specifically the  %\href{https://en.wikipedia.org/wiki/Category:Mathematical_puzzles}{Mathematical Puzzles}, only has Towers of Hanoi
    \href{https://en.wikipedia.org/wiki/Category:Logic_puzzles}{Logic Puzzles} category, the 
    \href{https://en.wikipedia.org/wiki/List_of_unsolved_problems_in_mathematics}{List of unsolved problems in mathematics}, and the
    \href{https://en.wikipedia.org/wiki/List_of_algorithms}{List of algorithms}.
    \item Programming competitions, including the [add links]International Collegiate Programming Contest and \href{https://codeforces.com}{codeforces.com}.
    \item The International Mathematical Competition (IMO) [add link], a high school competition
\end{itemize}

\paragraph{Translation.} Some problems can be converted to a \puzzle in a fairly straightforward process. For example, for the Towers of Hanoi problem, we chose a representation for the solution as a sequence of move pairs of integers $(i, j) \in \{0,1,2\}^2$ indicating a move from tower $i$ to tower $j$. In other cases, the conversion can be done but is not entirely obvious. For example, one way to define a compression puzzle is to give a decompression algorithm $d(x)$, a string $s$, and a target length $l$, and the puzzle is to find $x$ of length at most $l$ such that $d(x)=s$. For the classic Lempel-Ziv decompression algorithm, the decompression algorithm is defined in just six lines of python.

\paragraph{Solutions}. Each puzzle has 0-3 solutions, with the vast majority of puzzles have one solution. First, these solutions are helpful for debugging a \puzzle, just as programming competitions generally have one or more tested solutions to any problem. Second, these solutions can be used for training though care has to be taken to avoid ``contaminating'' the training with solutions to training problems related to test problems that give away the solution. To make it easier to avoid such contamination, the dataset is divided into files by category so that such related problems should all be in the same file.

\paragraph{Trivial \puzzles.} For most programming constructs, it is quite simple to define puzzles that test elementary language understanding. For example, \pyline{(lambda x: x + " world" == "Hello world")} is a simple puzzle testing comprehension of concatenation.

\subsection{Dataset statistics}


\textbf{We should have code that autogenerates a table for this section}


==> ignore/sections/experiments.tex <==
\section{Experiments}

We design our experiments to answer the following research questions:
\begin{enumerate}
    \item Extrapolation: Can solutions to easier \puzzle{}s guide models to solve harder ones?
    \item Interpolation: Can models that find a solution to one instance of a puzzle, easily solve other instances of the same puzzle?
    \item Do humans and models agree on the difficulty level of different puzzles?
\end{enumerate}

==> ignore/sections/intro.tex <==
\section{Introduction}
% par1: recent developments in ML lead to impressive results on many tasks. Yet it is unclear how much of the success is due to pattern matching and memorization and how much is due to fundamental reasoning capacities.

% par2: challenges and puzzles are great because they require thinking and, unless seen before, cannot be solved by memorization or intuition alone. Studies how shown that they are useful for teaching blah blah..

% par3: In this paper, we use puzzles to evaluate AI model's ability to reason (and to train them to do so?). Importantly, we develop a unified framework based on Python that supports any NP problem and is easy to use with contemporary models. 

% par4: We demonstrate the value of our framework by writing a large amount of known and new challenges.

% par5: our experiments...

% to conclude


Over time, certain AI challenges have tantalized programmers who could solve them without a computer but had no idea how to program a computer to do the same. Prior examples included playing chess or Go, and distinguishing images of cats vs.~dogs. A current such challenge is solving problems that involve designing and implementing algorithms. Today, computers factor numbers better than any human, but the code behind the vast majority of algorithms is written by humans and not AI. In particular, \textit{algorithmic problem solving}---the aspect of problem solving that requires formulating algorithms---is an interesting aspect of programming in which humans outperform computers.  

How can AI beat world chess and Go champions and yet not be able to solve programming competition problems designed for novices? One obstacle is the lack of objective evaluation that could measure incremental progress in algorithmic problem solving. AI chess performance was measured through chess matches and datasets such as ImageNet quantified image classification progress. We propose Programming Puzzles (\puzzle{}s) as a framework for measuring progress on algorithmic problem solving. 

A \puzzle{} is specified by a short program $f$ and a time bound $T$, and a \textit{solution} is an input $x$ which makes $f$ output \pyline{True} (in time $\leq T$). Viewing $f$ as a function, the goal is to find $x$ such that $f(x)=1$. For example, \pyline{x = "Hello"} solves the trivial \puzzle $f=$\pyline{(lambda x: x + " world" == "Hello world")}. Arguably, a beginning python programmer \textit{understands} $f$ more deeply in that they can find solve $f$, even though a computer can compile and evaluate %almost\footnote{In computing \pyline{f(0)} for \pyline{f = lambda n: 10 ** 10 ** n == 10 ** 10 ** 100} which involves computing googleplex, the universe is predicted to freeze over before a standard python interpreter would finish.} any 
\puzzles orders of magnitude faster and more accurately than any human. Many problems admit multiple distinct solutions, and, like short theorems requiring long proofs, short \puzzles may require long solutions. Also, note that the time bound $T$ does not account for the time spent solving the problem, which is bounded separately by $S$. Figure \ref{fig:simple} illustrates some challenges, including difficult ones that are unsolved by humans. As we shall see, humans today vastly outperform AI at \puzzle{}s. We now elaborate on some important aspects of \puzzle{}s.

% \paragraph{Programs as specifications.}

\paragraph{NP-completeness.}
It is easy to check if a given $x$ solves a given \puzzle{} by simply evaluating $f(x)$. Formally, the class of such problems is referred to as NP and it is easy to prove that \puzzle{}s are NP-complete: the Boolean Satisfiability problem (SAT) is NP-complete and any Boolean SAT formula such as $(x_0 \vee \neg x_7) \wedge \ldots$ can trivially be rewritten as a PP, e.g., 
\pyline{lambda x: (x[0] or not x[7]) ...}. The size of $f$ and time $T$ needed to evaluate it are both linear in the formula size. A common misconception is that all NP-complete problems are all equally intractable, but the theory of NP-completeness only speaks to the worst-case complexity of solving all \puzzle{}s. While any of our \puzzle{}s could theoretically be converted a mammoth Boolean SAT formula without any abstraction or intuition, such a formula may not be tantalizing. Anything that can be written as a SAT problem can generally be written more easily and more succinctly as a \puzzle{}, because \puzzle{} authoring involves coding in a traditional programming language rather than in Boolean formulas. 

\paragraph{The dataset.} This paper introduces an open-source dataset called \thedataset that encodes numerous classic algorithmic programming challenges, from the Towers of Hanoi which has long been used to teach the concept of recursion, to algorithmic problems such as shortest path, to longstanding open problems such as learning parity with noise or finding a cycle in the $3n+1$ process, which would disprove the Collatz conjecture. The \puzzle{}s were created by inspired by sources such as Wikipedia and programming competitions. While all the code in the current repository was written by the the paper authors (often inspired by other sources), we welcome contributions to this dataset. Contributing involves writing a puzzle checker, an instance generator if there is to be more than one instance, and a solver program (except for unsolved puzzles). A new entry here can be synthesized in minutes from a contributor's own imagination. As is the case with designing other types of puzzles, creativity is required to design challenges that require cleverness to solve. However, even mundane challenges can be useful for evaluation on the lower-end of the spectrum.

\paragraph{Solving instances vs.~algorithms.} The \puzzle{}s in our dataset are each an \textit{instance} of an algorithmic programming challenge, which can be solved in any language or output by a neural network. In particular, an AI can solve some instances without necessarily discovering an algorithm that solves every instance. For example, finding a factor of a given integer is different than finding an algorithm that factors all integers. In fact, an AI may discover that 2/3 of uniformly random 64-bit integers have 2 or 3 as a factor and therefore make substantial progress on the uniform-factoring puzzles in \thedataset. However, it would fail on \thedataset's huge factoring puzzles that use publicly-available numbers that have had prizes of hundreds of thousands dollars for solving. While it would be preferable to find general-purpose algorithms, puzzle instances facilitate easy evaluation with incremental progress in contrast to the notoriously difficult problem of testing program correctness.

\paragraph{Are puzzles enough to measure algorithmic problem solving?} Only some algorithmic problems make good puzzles. Unfortunately, ``soft'' challenges involving natural language or images are not naturally writable as \puzzles due to the ``glass-box'' \citep{christakopoulou2018glass} rather than black-box nature of \puzzles. This requirement, inherent to any NP problem,  would prohibit the hidden test sets necessary for evaluating such fuzzy ML problems. The breadth of problems in \thedataset illustrates the scope of \puzzles---in particular it is larger than that SAT which has found numerous applications over decades of study. Furthermore, as a means of evaluating algorithmic problem solving ability, one does not necessarily need to cover every type of algorithmic problem. If AI reaches human-level performance on \thedataset, then more general problems can be considered. 





A Program Reasoning Challenge is specified by We find these challenges to be a convenient way to test a variety of reasoning abilities. We introduce a dataset of python challenges that includes:
\begin{itemize}
    \item Classic puzzles: \href{https://en.wikipedia.org/wiki/Tower_of_Hanoi}{Towers of Hanoi}, \href{https://en.wikipedia.org/wiki/Verbal_arithmetic}{Verbal Arithmetic} (e.g., $\mathrm{SEND} + \mathrm{MORE} = \mathrm{MONEY}$), etc.
    \item Solitaire problems: the \textit{Game of Life} (e.g., finding oscillators of a given period) and \textit{Chess problems} (e.g., knight's tour problem)
    \item Solving two-player games: optimal strategies for \textit{Tic-Tac-Toe}, \textit{Rock-Paper-Scissors}, and zero-sum bimatrix games (equivalent to linear programming); finding Nash equilibria of general-sum games (PPAD complete), and finding winning strategies for \textit{Mastermind} and \textit{Connect Four}
    \item Problems inspired by programming and math competitions: \url{codeforces.com}, the International Mathematical Olympiad (IMO) and the International Collegiate Programming Contest (ICPC) 
    \item Graph-theory: algorithmic challenges such as finding the shortest path or finding a planted clique
    \item Elementary algebra: finding roots of quadratic, cubic and higher degree polynomials
    \item Number-theory: algorithmic challenges from GCD (solved by Euclid's algorithm) to factoring and discrete logarithm (open)
    \item Lattices: algorithmic challenges such as learning parities (solved by Gaussian elimination) or learning parity with noise (open)
    \item Compression: compressing (resp., decompressing) a given string given only the decompression (resp., compression) algorithm
    \item Open mathematics problems: Conway's 99-graph problem or finding a cycle in the Collatz process
\end{itemize}




% The Boolean satisfiability problem (SAT) has inspired decades of progress in optimization and theoretical computer science. %A SAT problem has the convenient verifiability property so that it does not need to be accompanied by a hidden test set. 
% Like any NP-complete problem, any other P or NP problem can be converted to SAT and it is not believed to be possible to efficiently solve \textit{all} SAT problems. Nonetheless, SAT solvers have proven useful in numerous commercial applications [add ref], as well as in AI research, e.g., Automatic Theorem Proving (ATP) [add ref] and specification-based program synthesis [add ref]. Nonetheless, SAT remains more of an optimization tool than an AI challenge, though ML has been used to improve SAT solvers [add ref].



% \paragraph{AI-SAT vs.~SAT:}
% both are NP complete and thus in theory problems can be converted between the two representations, with a trivial conversion from SAT to AI-SAT (see Figure ADD). However, there are multiple reasons why AI-SAT may be more suited to AI research than SAT. First, converting any NP problem to a AI-SAT involves writing a program to test a candidate solution while the conversion to an SAT formula is often more cumbersome, longer, and obfuscates the original problem. Unlike Boolean formulas, programming languages are designed to make it easy for humans to formalize common problems. Second, the lack of human intuition for how to solve SAT problems is an obstacle to AI research, and computers already outperform humans who have no chance of solving SAT formulas with millions of terms. On the other hand, SAT solvers have been improved over decades, and the syntax and semantics of Boolean formulas is much simpler than python programs. 



% This paper introduces a dataset of \textit{program satisfaction problems} which bridges the two domains. A program satisfaction problem is described by a program and the goal, like SAT, is to find an input which makes the program output \pyline{True}. An easy example problem is:
% \begin{lstlisting}[language=Python,basicstyle=\ttfamily]
%     def sat(s: str): # find a string with 1 occurrence of "aa" and 1000 occurrences of "a"
%         return s.count("aa") == 1 and s.count("a") == 1000
% \end{lstlisting}
% A human who knows python should generally be able to solve this, one solution being \pyline{"aa" + "ab"*999}, where in python string addition and multiplication correspond to concatenation and repetition, respectively. The goal is, given the program source, to find a program that outputs an input making the program return \pyline{True}. Of course, program satisfaction problems may be written in any programming language, but we choose python for our AI-SAT dataset given its pervasiveness in the AI community.  (In the implementation, the problem reads the input from a file so that the solver program can be written in any human programming language--or a neural network could directly output the answer.) A more challenging problem is:
% \begin{lstlisting}[language=Python,basicstyle=\ttfamily]
%     def sat(n: str): # find a string with 1 occurrence of "aa" and 1000 occurrences of "a"
%         return s.count("aa") == 1 and s.count("a") == 1000
% \end{lstlisting}


% AI-SAT problems have the following properties:
% \begin{enumerate}
%     \item While a problem may have be multiple correct solutions, one can trivially test solutions by evaluating the program. 
%     \item 
% \end{enumerate}


% Much, if not most work in the field of program synthesis is based entirely on example input-output pairs. While this has proven useful in some applications such as Flash Fill for Excel (add citation), Programming by Example has a few limitations: (a) advanced human programming problems like algorithms (e.g., SVD) or programming contest problems are not defined exclusively by examples, (b) 


% highlights the (current) superiority of human programmers over program synthesis systems at algorithm design. It has the following properties:
% \begin{enumerate}
%     \item Solutions can be \textit{machine-verified} meaning that a solver can easily verify its own solutions without needing to match a subjective solution in an answer key, without needing to understand a natural language such as English, and without needing to know about real-world concepts such as names, months, or animals.
%     \item It has programming problems ranging from easy to hard that involve abstract reasoning. These include elementary puzzles, programming competition problems, and even long-standing open problems in computer science and mathematics, the solution to some of which have been offered hundreds of thousands of dollars in monetary rewards.
% \end{enumerate}


\begin{figure}
\begin{pyblock}
def f(s: str): # hello world example
    return s + "world" == "Hello world"
    
def f(n: int, square=81):
    return n * n == square and n < 0

def f(s: str): # find a string with 100 a's but no two consecutive a's
    return s.count("a") == 100 and s.count("aa") == 0

\end{pyblock}
    \caption{Any spec that can be verified by a Turing machine in time $T$ can be encoded poly$(T)$-sized PP or SAT since both problems are NP-complete. Any SAT problem can be encoded as a PP of linear size.  However, the translation from the \lstinline[language=Python,basicstyle=\ttfamily]{easy} PP requires a SAT formula with millions of terms, obfuscating the obvious solution during translation. }
    \label{fig:examples}
\end{figure}
    
% def hanoi(moves: List[Tuple[int, int]]): 
%     state = ([8, 7, 6, 5, 4, 3, 2, 1], [], [])
%     for (i, j) in moves: # move (i, j) means move disk from rod i to rod j
%         state[j].append(state[i].pop())
%         assert state[j][-1] == min(state[j]), "larger disk on top of smaller disk"
%     return state == ([], [], [8, 7, 6, 5, 4, 3, 2, 1]
    
% def f(quine: str): # find a a program that evaluates to itself
%     return eval(quine) == quine

% def greater_common_divisor(divisor: int, m=153, n=85, lb=10): 
%     return m % divisor == 0 == n % divisor and divisor > lb
    


% def f6(seq: List[int], length=17, text="Hellooooooooooooooooooooo world!"): # LZH
%     index = [chr(i) for i in range(256)]
%     pieces = [""]
%     for i in seq:
%         pieces.append(pieces[-1] + pieces[-1][0] if i == len(index) else index[i])
%         index.append(pieces[-2] + pieces[-1][0])
%     return "".join(pieces) == text and len(seq) <= length

% def f7(li: List[int], n=3, colors=[0, 1, 2, 0, 0, 1, 1, 1, 2, 2, 0, 2]): # 2020 IMO \#3
%     assert len(li) == len(set(li)) and min(li) >= 0 and sum(li) * 2 == sum(range(4 * n))
%     return sorted([colors[i] for i in li]) == [i // 2 for i in range(2 * n)]

% def f8(factor: int, n=123456789): # find a non-trivial factor (hard for large n)
%     return 0 < factor < n and n % factor == 0
    
% def f9(edges: List[List[int]]): # Conway's 99 graph, open math problem 
%     N = {i: {j for j in range(99) if j != i and ([i, j] in edges or [j, i] in edges)} 
%             for i in range(99)}  # neighbor sets
%     return all(len(N[i].intersection(N[j])) == (1 if j in N[i] else 2) 
%               for i in range(99) for j in range(i))

% def f10(n: int): # Find a cycle in the Collatz process, longstanding open math problem
%     m = n
%     while n != 1:
%         n = 3 * n + 1 if n % 2 else n // 2
%         if n == m:
%             return m > 0




The NP-complete Boolean Satisfiability (SAT) problem, e.g., solving formulas like $(x_1 \vee x_2) \wedge (\neg x_1 \vee \neg x_2)$, has played a central role in optimization and computational complexity theory, and has had numerous applications within AI [add]. The PP problem also NP-complete. Thus, any efficiently verifiable problem spec can be converted to either a SAT problem or a PP. However, conversion to SAT is a laborious and niche skill, while writing a PP can be done by anyone who knows how to program -- one simply writes a program that checks a solution. Figure \ref{fig:sat} illustrates how any SAT formula can be trivially expressed as Python PP while a trivial PP may require an inscrutable SAT formula with millions of clauses.


\begin{figure}
\begin{lstlisting}[language=Python,frame=single,basicstyle=\ttfamily]
def sat(x: List[bool]): # PRC version of SAT formula $(x_1 \vee x_2) \wedge (\neg x_1 \vee \neg x_2)$
    return (x[0] or x[1]) and (not x[0] or not x[1]]) 
    
def easy(n: int): # PRC whose SAT encoding has millions of terms
    return str(2 ** n) == str(2 ** 345678)  # 2 ** n = $2^n$, str is string encoding
\end{lstlisting}
    \caption{Any spec that can be verified by a Turing machine in time $T$ can be encoded poly$(T)$-sized PP or SAT since both problems are NP-complete. Any SAT problem can be encoded as a PP of linear size.  However, the translation from the \lstinline[language=Python,basicstyle=\ttfamily]{easy} PP requires a SAT formula with millions of terms, obfuscating the obvious solution during translation. }
    \label{fig:sat}
\end{figure}





Our main contributions:
\begin{itemize}
    \item A new framework to evaluate reasoning capabilities of AI models with several desirable properties.
    \item A large set of diverse challenges with different difficulties.
    \item We evaluate several baselines
    \item Compare to human performance
\end{itemize}

==> ignore/sections/related.tex <==
\section{Related Work}

==> ignore/sections/solvers.tex <==
\section{Examined Solvers}
\tal{If we include GPT, maybe we'll have a different section for language models?...}

In this section, we describe the models we develop as baselines for the \thedataset dataset. 
\tal{probably this is too detailed. Can move some to the appendix.}

\paragraph{Task definition.}
We define a solver as a function $g: \mathcal{F} \rightarrow \mathcal{X}$ that given a puzzle $f \in \mathcal{F}$, returns a value $x \in \mathcal{X}$ that satisfies $f$ (i.e., \pyline{f(g()) == True}) in time $\le T$. We keep the specifics of $g$ abstract as it can be implemented in any language, as long as the output is converted to Python for evaluation. Furthermore, for a given puzzle $f$, the space of correct solutions $\mathcal{S}_\mathcal{F}$ is infinite. Specifically, correct solutions can either implement a solving strategy or keep the logical process hidden and directly return the answer. For example, if $f$ asks to find the shortest past between two nodes in a given graph, $g$ can either implement Dijkstra's algorithm to compute the path, or simply return the final answer (e.g., \pyline{return \[1, 5, 8\]}) without revealing the strategy. However, for some puzzles, the direct answer can be extremely long (e.g., \pyline{print([i/2 for i in range(10**6)])}). Nevertheless, Both options can be evaluated with our framework as we readily verify their absolute correctness by executing the code. This is an advantage over other text generation tasks that require prior annotation of reference solutions.

\paragraph{Solution decoding.}
Inspired by recent work~\citep{balog2016deepcoder, christakopoulou2018glass}, we develop models to guide the search for $g$ over the space of all possible functions. Following \citet{christakopoulou2018glass}, we implement a Domain Specific Language (DSL) on top of Python to make it type-safe and limit the search space and control the generation. Specifically, each Python function is translated to a tree of rules $R \in \mathcal{R}$. Each rule represents a specific Python operation and the types of the variables used in it.\tal{Adam, maybe you know how to explain this better}.
In order to guide the generation of $g$, we want to assign a probability for each rule to be used. The score of a program is then computed as the joint probability of all the rules used in it, and the solutions can be sorted accordingly. Naturally, this scoring mechanism introduces a bias towards shorter programs (i.e., smaller trees), which is desirable as generally we would prefer a shorter solution.

% copy
Since many solutions copy certain values of phrases from the puzzle, we add a \pyline{COPY} rule to our vocabulary. In run time, the rule is replaced with the simple identity function (\pyline{lambda x: x}). When composing the solution, this rule can reduce the complexity of the solution by simply learning to copy part of the puzzle rather than having to generate it from scratch. For simplicity, we create copy rules for each of the supported types and assign the probabilities uniformly across all the puzzle's phrases of that type. In other words, our models learn when a certain type should be copied from the puzzle, and rank all available phrases of that type the same.

\paragraph{Solution validation.}
\tal{should we say something about safe, timing etc?...}

\subsection{Models}
We evaluate three different models for predicting the rules in $g$. \tal{plus GPT and T-5?}

\paragraph{Uniform.}
The first model is a simple naive non-parametric uniform rule that assigns the same score for all rules. The only exception is the \pyline{COPY} rule, for which we allow the user to assign a fixed probability in order to bias the solver towards utilizing this option. As we score programs by their joint probability, essentially this results in preferring shorter programs. We use this model to find solutions to the easier problems that require a simple and short answer, that are used to bootstrap the learning of the parametric models. We also evaluate this model as a naive brute force solver and examine whether the supervised models can guide the solution search more efficiently.

\paragraph{Random Forest.}
Next, we implement a supervised bigram model to predict $\mathbb{P}(R_j|f, R_i, k)$ where $R_j$ is a candidate rule to appear in $g$'s tree under $R_i$ as its $k$'s argument. For this model we represent $f$ as a bag-of-rules $\sum_{R_i} \{R_i \in f\}$. Specifically, $f$ is featurized as a vector of length $|\mathcal{R}|$ representing the number of occurrences of each rule in $f$.\footnote{Since most of the values are zeros, we use sparse vectors.} $R_i$ and $k$ are encoded as a one-hot vector and concatenated to $f$'s representation to construct the input to the model. To train the model, we collect all parent-child rule pairs from available solutions to puzzles and fit a random forest with one hundred trees to predict each child rule from its parent. At inference, for a new puzzle, we apply the model over all rules in $\mathcal{R}$, mask out child rules that do not output the matching type, and re-normalize the scores to create a valid probability distribution. Then the solver iterates over solutions by their likelihood until it finds a solution $g$ s.t.\ \pyline{f(g())==True} in time $\le T$, for a maximum number of tries $M$.

\paragraph{Transformer.} 
Following the recent success of Transformer models~\citep{transformer2017} in encoding source code~\cite[\emph{inter alia}]{feng-etal-2020-codebert,Svyatkovskiy_2020,cubert}, we turn to these encoders to obtain a richer representation. We keep the bigram setting of the Random Forest setting (i.e., predicting a child rule from its parent), but use a Transformer to encode the puzzle $f$ and the candidate rules. 

\begin{figure}[t]
    \centering
    \includegraphics[width=0.5\textwidth]{figures/transformer.pdf}
    \caption{An illustration of our Transformer-based solver. The rule strings are encoded with a Transformer pretrained on Python code. The puzzle Transformer is initialized the same, but is further fine-tuned on or puzzles, together with the rest of solver's new parameters shown in blue color.}
    \label{fig:transformer}
\end{figure}

We use the RoBERTa-base 12-layers Transformer~\citep{liu2019roberta} pretrained on English text and fine-tune it on Python code using the Hugging Face library~\citep{wolf-etal-2020-transformers}. For fine-tuning data, we use Python functions with their documentation text from GitHub repositories~\citep{husain2019codesearchnet}. In order to better adjust the tokenizer to Python code, we retrain a Byte-level BPE tokenizer on our Python fine-tuning data. We use the same vocabulary size as the original tokenizer and keep the token embeddings of the overlapping ones (39\%). For the other tokens, we initialize new token embeddings. Thereafter, we fine-tune RoBERTa with a masked language modeling task for 30 epochs. We call this model $T_P$\tal{different notation?}. $T_P$ achieved an impressive $3.3$ perplexity score on held-out evaluation data, indicating its success in learning Python's syntax.

Next, we use $T_P$ to encode dense embeddings $e_R = T_P(R)$ for all the rules $R$ in our vocabulary $\mathcal{R}$. As input to the Transformer, we use a string representation of the Python operation and types of each rule. For example, \pyline{(x)//(y)' '// -> FLOAT :: (x: INT, y: FLOAT)} is used to describe the rule for the \pyline{//} operation with an integer and float inputs, resulting in a float. Then, we take $e_R$ as the average across the top-layer embeddings of all tokens. 

Finally, we design a neural model on top of $T_P$ to predict $\mathbb{P}(R_j|f, e_{R_i}, k)$. The model computes a hidden representation of the puzzle with the parent rule as a concatenation $h=[T_P(f), \mathbf{W}_1 e_{R_i}, e_k] \in \mathbb{R}^{d+d_r+d_k}$, where $e_k \in \mathbb{R}^{d_k}$ is a learned embedding for the child rule index, $\mathbf{W}_1 \in \mathbb{R}^{d_r}$ is a learned linear projection, and $d$ is the hidden dimension of $T_P$. Here, we use the $\texttt{[CLS]}$ embedding of the top layer as $T_P(f)$ and further fine-tune $T_P$ while keeping the rule embeddings $e_R$ fixed to prevent overfitting to the rules seen in the puzzle-solution training pairs. $h$ is then passed through two non-linear layers, where the first also projects it to $\mathbb{R}^{d_r}$, with a gelu activation~\citep{hendrycks2016gaussian} and batch normalization~\citep{ioffe2015batch} to get a joint puzzle and parent rule embedding $e_{f,{R_i},k}$. The score of rule $R_j$ then being the $k$ argument of $R_i$ in the solution to $f$ is determined by the dot product of its projected embedding $e_{R_j}$ with the parent's embedding: $p_{R_j|f, e_{R_i}, k} \propto  e_{f,{R_i},k} \cdot (\mathbf{W}_2 e_{R_j})^T$. Similar to the Random Forest fitting process, we use all parent-child rule pairs from the available solutions and use a cross-entropy loss with an Adam optimizer. 


% We develop several baseline solvers to experiment with the problems in our dataset. Our solvers vary in their complexity and in the way they encode the problems and decode the solutions. Since both problems and solutions are programs---or more concretely, functions---two typical representation options are as raw strings or as an Abstract Syntax Trees (AST). 

% The \emph{unstructured} string representation simply treats the program as a sequence of characters. One benefit of this approach is in its simplicity and flexibility, for example readily supporting comments and documentations. An unstructured autoregressive decoder, however, can result in syntax errors and requires long-term planning.



==> sections/app_gpt_outputs.tex <==

\section{GPT-3 Bootstrap results}\label{ap:gpt_examples}

Below are the 87 puzzles solved by the GPT-3 bootstrap run for 10K tries per puzzle on the set of 138 puzzles.

\begin{pylittledisplay}
# Bootstrap solved after 1 tries:
def f1(start: int, k=3, lower=150, seq=[3, 1, 2, 65, 18, 91, -30, 100, 0, 19, 52]):
    return 0 <= start <= len(seq) - k and sum(seq[start:start + k]) >= lower
SOL: "5"

# Bootstrap solved after 1 tries:
def f2(path: List[int], edges=[[0, 1], [0, 2], [1, 2], [1, 3], [2, 3]]):
    for i in range(len(path) - 1):
        assert [path[i], path[i + 1]] in edges
    assert path[0] == 0
    assert path[-1] == max(max(edge) for edge in edges)
    return True
SOL: "list(range(4))"

# Bootstrap solved after 2 tries:
def f3(n: int, s='0000111111100000', k=5):
    return s[n:n + k] == s[n] * k
SOL: "4"

# Bootstrap solved after 3 tries:
def f4(z: float, v=9, d=0.0001):
    return int(z * 1/d % 10) == v
SOL: "2.3"

# Bootstrap solved after 3 tries:
def f5(n: int, scores=[100, 95, 80, 70, 65, 9, 9, 9, 4, 2, 1], k=6):
    assert all(scores[i] >= scores[i + 1] for i in range(len(scores) - 1)), "Hint: scores are non-decreasing"
    return all(s >= scores[k] and s > 0 for s in scores[:n]) and all(s < scores[k] or s <= 0 for s in scores[n:])
SOL: "8"

# Bootstrap solved after 4 tries:
def f6(n: int, lace='bbbbrrbrbrbbrrrr'):
    sub = lace[n: n + len(lace) // 2]
    return n >= 0 and lace.count("r") == 2 * sub.count("r") and lace.count("b") == 2 * sub.count("b")
SOL: "4"

# Bootstrap solved after 7 tries:
def f7(i: int, s='cat', target='a'):
    return s[i] == target
SOL: "1"

# Bootstrap solved after 10 tries:
def f8(n: int, ops=['x++', '--x', '--x'], target=19143212):
    for op in ops:
        if op in ["++x", "x++"]:
            n += 1
        else:
            assert op in ["--x", "x--"]
            n -= 1
    return n == target
SOL: "19143213"

# Bootstrap solved after 11 tries:
def f9(n: int, target='foofoofoofoo', s='foofoo'):
    return s * n == target
SOL: "2"

# Bootstrap solved after 12 tries:
def f10(i: int, li=[17, 31, 91, 18, 42, 1, 9], target=18):
    return li[i] == target
SOL: "3"

# Bootstrap solved after 19 tries:
def f11(li: List[int]):
    return all(j in {i - 1, i + 1, 3 * i} for i, j in zip([0] + li, li + [128]))
SOL: "list(range(128))"

# Bootstrap solved after 20 tries:
def f12(n: int, year_len=365):
    prob = 1.0
    for i in range(n):
        prob *= (year_len - i) / year_len
    return (prob - 0.5) ** 2 <= 1/year_len
SOL: "24"

# Bootstrap solved after 23 tries:
def f13(si: Set[int]):
    return all(i in range(1000) and abs(i - j) >= 10 for i in si for j in si if i != j) and len(si) == 100
SOL: "set(range(1, 1000, 10))"

# Bootstrap solved after 25 tries:
def f14(ls: List[str]):
    return tuple(ls) in zip('dee', 'doo', 'dah!')
SOL: "['d', 'd', 'd']"

# Bootstrap solved after 30 tries:
def f15(start: int, k=3, lower=100000, seq=[91, 1, 2, 64, 18, 91, -30, 100, 3, 65, 18]):
    prod = 1
    for i in range(start, start + k):
        prod *= seq[i]
    return prod >= lower
SOL: "3"

# Bootstrap solved after 30 tries:
def f16(li: List[int], n=85012):
    return len(li) == n
SOL: "list(range(85012))"

# Bootstrap solved after 48 tries:
def f17(x: List[int], a=7, s=5, e=200):
    return x[0] == a and x[-1] <= e and (x[-1] + s > e) and all([x[i] + s == x[i+1] for i in range(len(x)-1)])
SOL: "list(range(7, 200, 5))"

# Bootstrap solved after 57 tries:
def f18(item: int, li=[17, 2, 3, 9, 11, 11], index=4):
    return li.index(item) == index
SOL: "11"

# Bootstrap solved after 64 tries:
def f19(start: int, k=3, upper=6, seq=[17, 1, 2, 65, 18, 91, -30, 100, 3, 1, 2]):
    return 0 <= start <= len(seq) - k and sum(seq[start:start + k]) <= upper
SOL: "8"

# Bootstrap solved after 79 tries:
def f20(x: List[int]):
    return len(x) == 2 and sum(x) == 3
SOL: "[] + [1, 2]"

# Bootstrap solved after 119 tries:
def f21(s: str, n=7):
    return int(str(5 ** n)[:-2] + s) == 5 ** n
SOL: "str(int(-5) ** 2)"

# Bootstrap solved after 129 tries:
def f22(s: str):
    return float(s) + len(s) == 4.5
SOL: "str('1.5')"

# Bootstrap solved after 131 tries:
def f23(s: str):
    return "Hello " + s == "Hello world"
SOL: "str('world')"

# Bootstrap solved after 141 tries:
def f24(s: str, target='foofoofoofoo', n=2):
    return s * n == target
SOL: "str('foofoo')"

# Bootstrap solved after 145 tries:
def f25(s: str, a=['cat', 'dot', 'bird'], b=['tree', 'fly', 'dot']):
    return s in a and s in b
SOL: "str('dot')"

# Bootstrap solved after 151 tries:
def f26(s: str, target='foobarbazwow', length=6):
    return target[(len(target) - length) // 2:(len(target) + length) // 2] == s
SOL: "str('barbaz')"

# Bootstrap solved after 160 tries:
def f27(s: str):
    return s + 'world' == 'Hello world'
SOL: "str('Hello ')"

# Bootstrap solved after 162 tries:
def f28(x: str, s=['a', 'b', 'c', 'd', 'e', 'f'], n=4):
    return len(x) == n and all([x[i] == s[i] for i in range(n)])
SOL: "str('abcd')"

# Bootstrap solved after 162 tries:
def f29(st: str, a='world', b='Hello world'):
    return st + a == b
SOL: "str('Hello ')"

# Bootstrap solved after 166 tries:
def f30(li: List[int]):
    return li.count(17) == 3 and li.count(3) >= 2
SOL: "list([17, 3, 17, 3, 17])"

# Bootstrap solved after 177 tries:
def f31(s: str, strings=['cat', 'dog', 'bird', 'fly', 'moose']):
    return s in strings and sum(t > s for t in strings) == 1
SOL: "str('fly')"

# Bootstrap solved after 179 tries:
def f32(s: str, a='hello', b='yellow', length=4):
    return len(s) == length and s in a and s in b
SOL: "str('ello')"

# Bootstrap solved after 199 tries:
def f33(li: List[int]):
    return len(li) == 10 and li.count(li[3]) == 2
SOL: "list([0, 10, 0, 10, 0, 3, 1, 2, 6, 2])"

# Bootstrap solved after 221 tries:
def f34(n: int, nums=[15, 27, 102], upper_bound=5000):
    return all(n % i == 0 for i in nums) and n <= upper_bound
SOL: "0"

# Bootstrap solved after 231 tries:
def f35(s: str, n=1000):
    return len(s) == n
SOL: "str('f' * 1000)"

# Bootstrap solved after 237 tries:
def f36(x: int, a=93252338):
    return -x == a
SOL: "int(-93252338)"

# Bootstrap solved after 269 tries:
def f37(x: int, a=-382, b=14546310):
    return x - a == b
SOL: "int(14546310 - 382)"

# Bootstrap solved after 301 tries:
def f38(x: int, a=8665464, b=-93206):
    return a - x == b
SOL: "int(8665464 - -93206)"

# Bootstrap solved after 302 tries:
def f39(i: int, s='cat', target='a'):
    return s[i] == target and i < 0
SOL: "int(-2)"

# Bootstrap solved after 321 tries:
def f40(x: int, a=9384594, b=1343663):
    if x > 0 and a > 50:
        return x - a == b
    else:
        return x + a == b
SOL: "int(9384594 - -1343663)"

# Bootstrap solved after 325 tries:
def f41(i: int, li=[17, 31, 91, 18, 42, 1, 9], target=91):
    return li[i] == target and i < 0
SOL: "int(-5)"

# Bootstrap solved after 336 tries:
def f42(s: str):
    return s[::-1] + 'world' == 'Hello world'
SOL: "str('Hello ')[::-1]"

# Bootstrap solved after 341 tries:
def f43(s: str):
    return "Hello " + s[::-1] == "Hello world"
SOL: "str(\"dlrow\")"

# Bootstrap solved after 342 tries:
def f44(n: int, a=14302, b=5):
    return b * n + (a % b) == a
SOL: "int(14302 / 5)"

# Bootstrap solved after 350 tries:
def f45(x: int, a=253532, b=1230200):
    if x > 0 or a > 50:
        return x - a == b
    else:
        return x + a == b
SOL: "int(253532 + 1230200)"

# Bootstrap solved after 385 tries:
def f46(x: int, a=4, b=54368639):
    if a == 1:
        return x % 2 == 0
    elif a == -1:
        return x % 2 == 1
    else:
        return x + a == b
SOL: "int(54368639 - 4)"

# Bootstrap solved after 398 tries:
def f47(li: List[int]):
    return li[li[0]] != li[li[1]] and li[li[li[0]]] == li[li[li[1]]]
SOL: "list([3, 9, 9, 4, 1, 9, 8, 6, 1, 10, 1, 9])"

# Bootstrap solved after 402 tries:
def f48(n: int, a=3, b=23463462):
    return b // n == a
SOL: "int(23463463 / 3)"

# Bootstrap solved after 451 tries:
def f49(x: int, a=1073258, b=72352549):
    return a + x == b
SOL: "int(72352549 - 1073258)"

# Bootstrap solved after 462 tries:
def f50(li: List[int]):
    return all([li[i] != li[i + 1] for i in range(10)]) and len(set(li)) == 3
SOL: "list([9, 1, 0, 9, 1, 0, 9, 1, 0, 9, 1, 0])"

# Bootstrap solved after 488 tries:
def f51(n: int, a=15482, b=23223, lower_bound=5):
    return a % n == 0 and b % n == 0 and n >= lower_bound
SOL: "int(23223 / 3)"

# Bootstrap solved after 488 tries:
def f52(n: int, nums=[77410, 23223, 54187], lower_bound=2):
    return all(i % n == 0 for i in nums) and n >= lower_bound
SOL: "int(23223 / 3)"

# Bootstrap solved after 493 tries:
def f53(li: List[int], target=[17, 9, -1, 17, 9, -1], n=2):
    return li * n == target
SOL: "list([17, 9, -1])"

# Bootstrap solved after 504 tries:
def f54(path: List[int], edges=[[0, 2], [0, 1], [2, 1], [2, 3], [1, 3]]):
    assert path[0] == 0 and path[-1] == max(max(e) for e in edges)
    assert all([[a, b] in edges for a, b in zip(path, path[1:])])
    return len(path) % 2 == 0
SOL: "list([0, 2, 1, 3])"

# Bootstrap solved after 539 tries:
def f55(e: List[int], edges=[[0, 217], [40, 11], [17, 29], [11, 12], [31, 51]]):
    return e in edges
SOL: "list([40, 11])"

# Bootstrap solved after 652 tries:
def f56(n: int, a=345346363, b=10):
    return n // b == a
SOL: "int(3453463634)"

# Bootstrap solved after 758 tries:
def f57(path: List[int], edges=[[0, 11], [0, 22], [11, 22], [11, 33], [22, 33]], u=0, v=33, bound=3):
    assert path[0] == u and path[-1] == v and all([i, j] in edges for i, j in zip(path, path[1:]))
    return len(path) <= bound
SOL: "list([0, 22, 33])"

# Bootstrap solved after 782 tries:
def f58(p: List[int], edges=[[0, 1], [0, 2], [1, 2], [3, 1], [2, 3]]):
    return p[0] == 0 and p[-1] == 1 == len(p) % 2 and all([[a, b] in edges for a, b in zip(p, p[1:])])
SOL: "list([0, 1, 2, 3, 1])"

# Bootstrap solved after 787 tries:
def f59(s: str, dups=2021):
    return len(set(s)) == len(s) - dups
SOL: "str(2022 * 'S')"

# Bootstrap solved after 846 tries:
def f60(x: str, s=679):
    return s == sum([int(d) for d in x])
SOL: "str('1' * 679)"

# Bootstrap solved after 1039 tries:
def f61(li: List[int]):
    return all(sum(li[:i]) == 2 ** i - 1 for i in range(20))
SOL: "list(map(lambda i: 2**i, range(20)))"

# Bootstrap solved after 1043 tries:
def f62(x: int, a=10201202001):
    return x ** 2 == a
SOL: "int(10201202001 ** 0.5)"

# Bootstrap solved after 1053 tries:
def f63(probs: List[float]):
    assert len(probs) == 3 and abs(sum(probs) - 1) < 1e-6
    return max(probs[(i + 2) % 3] - probs[(i + 1) % 3] for i in range(3)) < 1e-6
SOL: "list(map(lambda i: float((i + 2) / 3 - (i + 1) / 3), range(3)))"

# Bootstrap solved after 1059 tries:
def f64(x: List[int], t=50, n=10):
    assert all([v > 0 for v in x])
    s = 0
    i = 0
    for v in sorted(x):
        s += v
        if s > t:
            return i == n
        i += 1
    return i == n
SOL: "list([12, 4, 3, 1, 2, 1, 5, 94, 2, 2, 13])"

# Bootstrap solved after 1121 tries:
def f65(x: float, a=1020):
    return abs(x ** 2 - a) < 10 ** -3 and x < 0
SOL: "float(-1020 ** 0.5)"

# Bootstrap solved after 1147 tries:
def f66(x: float, a=1020):
    return abs(x ** 2 - a) < 10 ** -3
SOL: "float(1020 ** 0.5)"

# Bootstrap solved after 1282 tries:
def f67(n: int, a=10000200001):
    return a == n * n and n < 0
SOL: "int(-10000200001 ** 0.5)"

# Bootstrap solved after 1299 tries:
def f68(i: int, n=62710561):
    return 1 < i < n and n % i == 0
SOL: "int(62710561 ** 0.5)"

# Bootstrap solved after 1331 tries:
def f69(i: int):
    return len(str(i + 1000)) > len(str(i + 1001))
SOL: "int(-1001)"

# Bootstrap solved after 1375 tries:
def f70(li: List[int]):
    return all([sum(li[:i]) == i for i in range(20)])
SOL: "list([1] * 20)"

# Bootstrap solved after 1414 tries:
def f71(big_str: str, sub_str='foobar', index=2):
    return big_str.index(sub_str) == index
SOL: "str('f foobar foo f')"

# Bootstrap solved after 1669 tries:
def f72(x: int, a=324554, b=1345345):
    if a < 50:
        return x + a == b
    else:
        return x - 2 * a == b
SOL: "int(1345345 + 324554 * 2)"

# Bootstrap solved after 1752 tries:
def f73(s: str, strings=['cat', 'dog', 'bird', 'fly', 'moose']):
    return s[::-1] in strings and sum(t < s[::-1] for t in strings) == 1
SOL: "str('cat')[::-1]"

# Bootstrap solved after 1760 tries:
def f74(s: str):
    return s.count('o') == 1000 and s.count('oo') == 0
SOL: "str(\"ow\" * 1000)"

# Bootstrap solved after 2456 tries:
def f75(nums: List[int], target=10):
    assert target % 9 not in [4, 5], "Hint"
    return len(nums) == 3 and sum([i ** 3 for i in nums]) == target
SOL: "list([1, 1, 2])"

# Bootstrap solved after 2517 tries:
def f76(x: List[int], n=5, s=19):
    return len(x) == n and sum(x) == s and all([a > 0 for a in x])
SOL: "list([2, 7, 3, 1, 6])"

# Bootstrap solved after 3027 tries:
def f77(i: int):
    return i % 123 == 4 and i > 10 ** 10
SOL: "int(10 ** 10 * 123 + 4)"

# Bootstrap solved after 3388 tries:
def f78(s: str, big_str='foobar', index=2):
    return big_str.index(s) == index
SOL: "str('ob')"

# Bootstrap solved after 3447 tries:
def f79(ls: List[str]):
    return min(ls) == max(ls) == str(len(ls))
SOL: "['2', '2']"

# Bootstrap solved after 3890 tries:
def f80(li: List[int], dups=42155):
    return len(set(li)) == len(li) - dups
SOL: "list(range(42155))*2"

# Bootstrap solved after 5560 tries:
def f81(n: int):
    return str(n * n).startswith("123456789")
SOL: "int(int(\"123456789\" * 2) ** 0.5)"

# Bootstrap solved after 5986 tries:
def f82(ls: List[str]):
    return [s + t for s in ls for t in ls if s != t] == 'berlin berger linber linger gerber gerlin'.split()
SOL: "['ber', 'lin', 'ger']"

# Bootstrap solved after 6086 tries:
def f83(bi: List[int], g1=[[0, 1], [1, 2], [2, 3], [3, 4]], g2=[[0, 4], [4, 1], [1, 2], [2, 3]]):
    return len(bi) == len(set(bi)) and {(i, j) for i, j in g1} == {(bi[i], bi[j]) for i, j in g2}
SOL: "list([0, 2, 3, 4, 1])"

# Bootstrap solved after 6408 tries:
def f84(x: float):
    return str(x - 3.1415).startswith("123.456")
SOL: "float(123.456 + 3.1415)"

# Bootstrap solved after 6686 tries:
def f85(si: Set[int]):
    return {i + j for i in si for j in si} == {0, 1, 2, 3, 4, 5, 6, 17, 18, 19, 20, 34}
SOL: "set([0, 1, 2, 3, 17])"

# Bootstrap solved after 6849 tries: ("The Monkey and the coconuts" ancient puzzle)
def f86(n: int):
    for i in range(5):
        assert n % 5 == 1
        n -= 1 + (n - 1) // 5
    return n > 0 and n % 5 == 1
SOL: "int(10 ** 10 * 105 - 4)"

# Bootstrap solved after 8845 tries:
def f87(ls: List[str]):
    return ls[1234] in ls[1235] and ls[1234] != ls[1235]
SOL: "['foo', 'bar', 'foobar']*1234"  
\end{pylittledisplay}


==> sections/checklist.tex <==
\section*{Checklist}

% %%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
% %%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{as mentioned at the end of the introduction, our main contributions are (a) the puzzles framework; (b) the P3 dataset; and (c) evaluating baseline models.}
  \item Did you describe the limitations of your work?
    \answerYes{See Section~\ref{sec:the_dataset} and Conclusions: puzzles do not cover all types of challenges. Also, directly comparing human- and machine-performance is problematic so it depends on the available computational resources. Instead, we focus on the perceived difficulty.}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNo{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{}
	\item Did you include complete proofs of all theoretical results?
    \answerYes{} See Appendix \ref{sec:NP}
\end{enumerate}

\item If you ran experiments (e.g. for benchmarks)...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{See Appendix~\ref{sec:td_details}-\ref{sec:gpt3_details} for implementation details. We publicly share the data, and will privately share our baselines code with reviewers (we need to internally approve the code before publicly releasing).}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{See Appendix~\ref{sec:td_details}-\ref{sec:gpt3_details} for details. As are whole setting is unsupervised, we did not perform any hyperparameter tuning and use the same values aross model variants. The default values are provided in the running scripts with the code.}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{and [No]. See Appendix~\ref{sec:study_details} for analysis of the user study (specifically, Figures~\ref{fig:hack_yoe}-\ref{fig:user_study}). Figure~\ref{fig:cumsum} includes standard deviation for the enumerative models across three runs. We did not rerun the GPT-3 solvers more than once per setting yet.}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{See Appendix~\ref{sec:td_details}-\ref{sec:gpt3_details}}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerYes{See the linked GitHub repository.}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{See the linked GitHub repository in footnote 1, page 1.}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerYes{See the figures in \ref{sec:study_details}}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerYes{See \ref{sec:study_res} and \ref{sec:study_details} for details about the recruiting and agreement for the user study.}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerYes{See \ref{sec:study_res} and \ref{sec:study_details} for details about the recruiting and agreement for the user study.}
\end{enumerate}

\end{enumerate}

